Publishing statistical models: Getting the most out of particle physics experiments

The statistical models used to derive the results of experimental analyses are of incredible scientific value and are essential information for analysis preservation and reuse. In this paper, we make the scientific case for systematically publishing the full statistical models and discuss the technical developments that make this practical. By means of a variety of physics cases -- including parton distribution functions, Higgs boson measurements, effective field theory interpretations, direct searches for new physics, heavy flavor physics, direct dark matter detection, world averages, and beyond the Standard Model global fits -- we illustrate how detailed information on the statistical modelling can enhance the short- and long-term impact of experimental results.

==> Makefile <==
FILENAME = draft

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

LATEX = pdf 

BIBTEX = bibtex

default: text copy_draft

all: default

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn

clean_drafts:
	rm -f draft_*.pdf

realclean: clean
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: deep_clean text
	
	sed -i.bak 's/cache=false/cache=true/' $(FILENAME).tex
	$(MAKE) text
	
	mkdir submit_to_arXiv
	cp $(FILENAME).tex submit_to_arXiv
	cp *.bbl submit_to_arXiv/ms.bbl
	
	cp *.bst submit_to_arXiv
	cp orcidlink.sty submit_to_arXiv
	cp SciPost.cls submit_to_arXiv
	cp -r plots submit_to_arXiv
	cp -r code submit_to_arXiv
	cp Makefile submit_to_arXiv
	mv _minted-$(FILENAME) submit_to_arXiv/_minted-ms
	mv submit_to_arXiv/$(FILENAME).tex submit_to_arXiv/ms.tex
	
	
	sed -i.bak '/^ *
	
	
	sed -i.bak 's/finalizecache/frozencache/' submit_to_arXiv/ms.tex
	
	find submit_to_arXiv/ -name "*.bak" -type f -delete
	
	find submit_to_arXiv/ -name "*.bib" -type f -delete
	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean
	if [ -f $(FILENAME).tex.bak ];then \
		mv $(FILENAME).tex.bak $(FILENAME).tex; \
	fi

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv

